Physics-aware Roughness Optimization for Diffractive Optical Neural Networks

As a representative next-generation device/circuit technology beyond CMOS, diffractive optical neural networks (DONNs) have shown promising advantages over conventional deep neural networks due to extreme fast computation speed (light speed) and low energy consumption. However, there is a mismatch, i.e., significant prediction accuracy loss, between the DONN numerical modelling and physical optical device deployment, because of the interpixel interaction within the diffractive layers. In this work, we propose a physics-aware diffractive optical neural network training framework to reduce the performance difference between numerical modeling and practical deployment. Specifically, we propose the roughness modeling regularization in the training process and integrate the physics-aware sparsification method to introduce sparsity to the phase masks to reduce sharp phase changes between adjacent pixels in diffractive layers. We further develop $2\pi$ periodic optimization to reduce the roughness of the phase masks to preserve the performance of DONN. Experiment results demonstrate that, compared to state-of-the-arts, our physics-aware optimization can provide $35.7\%$, $34.2\%$, $28.1\%$, and $27.3\%$ reduction in roughness with only accuracy loss on MNIST, FMNIST, KMNIST, and EMNIST, respectively.

==> 2pi_optimize.tex <==
%{\color{red}I would like to show phase mask with/without roughness training, after block prune, after 2pi process and its roughness as caption}

{
% After applying the block sparsification in Section \ref{blk_prune}, 
% The roughness score of the phase mask could be higher 
As block sparsified pixels are all zeros while other pixels around the sparsified blocks can have high positive values, which results in larger roughness at the block sparsified pixels and its surrounding pixels as shown in Table \ref{mnist} -- \ref{emnist} and Fig. \ref{map}. Thus, we need post-processing for recovering the roughness.
% after block sparsification. 
% Thanks to the $2\pi$ period of the phase modulation in DONN system,
We observe that the phase modulation of light signal features with 2$\pi$ period, i.e., for a trained phase modulation $c \in [0, 2\pi]$, we have $f(c + 2\pi) = f(c)$, where $f$ is the forward function of the DONN system, which provides us the opportunity to smoothen the phase mask by adjusting the pixels in diffractive layers with $2\pi$ in DONN models. 
% as discussed in Section \ref{background:deploy}, 
Thanks to this characteristic, we can optimize the roughness of the phase mask by selectively adding $2\pi$ to each pixel without retraining as no performance change happens in the model inference. 

Specifically, we formulate the selection of adding $2\pi$
% or not 
to each pixel in diffractive layers as a combinatorial optimization (CO) problem, and solve it with Gumbel-Softmax (GS)~\cite{jang2016categorical} with gradient descent algorithm. 
In forward, for a phase mask with size of $200\times200$, we have a selection mask of $200\times200\times2$ for selecting the add-on phase of $0$ or $2\pi$ for each pixel in the phase mask, where the selection at each pixel is one-hot represented. Thus, with a matrix of $[[0], [2\pi]]$, by matrix multiplication between $200\times200\times2$ selection mask and the vector $[[0],[2\pi]]$ with size of $2\times1$, the resulting add-on phase mask is $200\times200\times1$ containing either $0$ or $2\pi$ as the add-on phase. The loss function is the roughness computed with the add-on phase and the original phase mask as discussed in Section \ref{roughness}. 

In
% the 
backward,
% optimization process, 
% where 
we minimize the roughness loss function. The GS algorithm makes the discrete one-hot represented selection differentiable with continuous approximation of discrete samples~\cite{jang2016categorical}. Specifically, starting from the loss function, it approximates the one-hot selection with continuous probability selection and update probability for the selection options with the backpropagated gradients. Thus, in the next iteration, the loss function is updated with the newly optimized selection probability.
}
%{\color{red} consider a illurstration figure of GS here.}

==> block_smooth.tex <==
% As block pruning is applied (shown in Section~\ref{blk_prune}), all the weights in the pruned blocks would be set to zero and the weights in the unpruned blocks would distributed irregularly.
Roughness modeling pushes the smoothness of the entire weight matrix in diffractive layers during training, while block sparsification partitions the weight matrix into blocks with all the weights in the sparsified blocks being set to zero and the weights in the unsparsified blocks being distributed irregularly.
To reduce the sharp phase changes in the unsparsified blocks, we perform intra-block smoothness, again with the premise that it is differentiable with the training process. As the example shown in Fig.~\ref{intra_rough}, the weight matrix of a diffractive layer is split into nine $2 \times 2$ blocks. Variance of each block is computed and summed together. The obtained summation is added to the DONN system loss function as the roughness as Equation~\ref{eq:intra_rough}.
\vspace{-0.1cm}
\begin{equation}
\label{eq:intra_rough}
\small
L = \parallel \text{Softmax}(I) - t \parallel_{2} + p \times R(\mathbf{W}) + q \times R_{intra}(\mathbf{W})
\vspace{-0.1cm}
\end{equation}
where $q$ is the regularization factor and $R_{intra}(\mathbf{W})$ is the summation of variance of each block in each diffractive layer. In this case, $\boldsymbol\ell_{r}(\mathbf{W}) = p \times R(\mathbf{W}) + q \times R_{intra}(\mathbf{W})$.

\begin{figure}[t]
\centering
  \includegraphics[width=0.6\linewidth]{fig/intra_rough.pdf}
\caption{Illustration of intra-smoothness for a sparsified phase mask with sparsification ratio being $0.33$, block size being $2$.}
\label{intra_rough}
% \vspace{-0.2cm}
\end{figure}


==> intro.tex <==
% Deep neural networks (DNNs) have shown significant growth in many fields in recent years such as image classification~\cite{}, large-scale object detection~\cite{}, and natural language processing~\cite{}. However, as the requirements for model accuracy increase, DNNs that are implemented on digital platforms are usually accompanied by large energy consumption, large memory footprint, long computation time, etc.
% As the layers of DNNs get deeper and model size of DNNs gets larger (e.g., ResNet-152~\cite{he2016deep} with 152 layers and 11.3 billion FLOPs), 

The high computation and memory storage of deep neural networks (DNNs) pose intensive challenges to the conventional Von-Neumann architecture~\cite{islam2022eve, peng2021binary, islam2022enabling}, introducing substantial data movements in memory hierarchy. The yearning for the ultra-efficient DNN accelerators has driven the studies on many different Von-Neumann architectures. We are in urgent need of (i) a next-generation device/circuit technology beyond CMOS and (ii) the corresponding customized algorithm-technology co-design to achieve ultra-low power, real-time DNN processing in various applications.


As a representative, diffractive optical neural networks (DONNs) has drawn much attention. DONNs realizes the all-optical processing based on the physical phenomena, i.e., light diffraction and light signal phase modulation, which happen by nature at the light speed. Weights are encoded as complex-valued transmission coefficients in diffractive layers, and the free-space propagation function~\cite{ersoy2006diffraction} is adopted to multiply with the light wave function to realize computation. Multiple layers of diffractive surfaces features millions of neurons and physically formed the neural network, which mimic the morphology of artificial neural network, while consuming significantly less energy compared to running conventional DNNs on digital platforms.
Therefore, we could achieve high system throughput and computation speed,
% with low power consumption meaning 
with no extra energy cost required for maintaining the function of the computation units (pixels in the phase mask) in DONN systems once the phase masks are fabricated or assembled~\cite{lin2018all, zhou2021large, li2021late, li2022physics, chen2022physics}.
% in the medium.
% without additional energy cost expect for the light source,
% on optical devices, 
% Specifically, we implement machine learning tasks 
% % Additionally, the DONNs
% % complete the ML-tasks
% by manipulating the phase information carried by the light signal, which can be realized by passive optical devices functioning as phase masks.
% is gradually being focused on. 
%DONNs provide a promising approach to replace artificial deep neural networks (DNNs) as they can effectively alleviate partial software and electronic hardware operations. %In DONNs, dense matrix multiplication, which is the most time and energy-consuming part of DNN, can be performed at the speed of light in the medium. 
% DONNs features with its high system throughput, inherent parallel processing and high computation speed at low power consumption by realizing the all-optical inference on passive optical devices \cite{lin2018all,chen2022physics,zhou2021large}. 
%DONNs features with its high system throughput, inherent parallel processing and high computation speed at low power consumption by realizing the all-optical inference on passive optical devices. 
% Specifically, DONNs function based on the physical phenomena, i.e., light diffraction and light signal phase modulation, which happen by nature at the light speed in the medium without additional energy cost expect for the light source. Additionally, the DONNs complete the ML-tasks by manipulating the phase information carried by the light signal, which can be realized by passive optical devices functioning as phase masks, which means no extra energy cost required for maintaining the function of the computation units (pixels in the phase mask) in DONN systems once the phase masks are fabricated or assembled.}

%\textcolor{red}{(Why ONN has zero power consumption? Show device picture proof.)}

%\textcolor{red}{(Problem of deployment of DONN.)} However, since the DONN system relies on the diffraction of light by optical devices, there is significant accuracy degradation when deploying the digitally trained DONN on the physical optical hardware if the practical response of the optical devices is not considered carefully. Interpixel interaction within phase masks (diffractive layers of DONN) can result in a fast-varying incident field, which breaks down the computed optical responses in DONN models. 

Current DONN systems for all-optical inference is trained on digital platforms with the numerical modelling of the DONN system. However, there is a \textit{mismatch}, i.e., significant prediction accuracy degradation, between numerical modelling and physical deployment.
% As a result, there is a significant performance degradation when deploying the digitally trained DONN on the physical optical hardware without considering the practical optical responses of optical components carefully. 
% Such mismatch could be caused by
%  between numerical modelling and physical deployment such as
Potential reasons of such mismatch are:
discrete control levels in optical devices~\cite{zhou2021large}, fabrication errors of devices~\cite{li2022rubikonns, chen2022physics, chen2022complex}, inaccurate emulation kernels~\cite{chen2022physics}, etc. Among them, we identify the interpixel crosstalk \cite{yariv1993interpage} within the phase mask as most critical~\cite{lou2023effects,vallone2018diffusive,o2004diffractive}\,
% in the deployment of DONNs can be a significant contributor, 
since it breaks down the emulated computed optical responses from numerical modelling, as the sharp changes between adjacent pixels will introduce a fast-varying incident field. Thus, the impacts of interpixel crosstalk can be quantified using adjacency pixel thickness differences, namely \textit{roughness}. % \textcolor{red}{(CD: can we link this description with roughness? I see some disconnection.)}

To narrow the accuracy gap between digital emulation and hardware deployment, in this paper, we propose a physics-aware roughness optimization process for the DONN system.
% , which combines roughness modeling regularization with physics-aware weight sparsification to reduce the interpixel interaction within the phase mask in DONN system. 
Specifically, our proposed physics-aware optimization process includes three steps (Table \ref{tbl:pruning_feature}): \textbf{(1)} integrating roughness regularization into DONN loss function during training. Details are illustrated in Section \ref{roughness}, where a regularization factor is introduced in the training loss for the roughness-aware DONN training; \textbf{(2)} compressing models with block sparsification,
% to introduce mask sparsity, 
which migrates interpixel interaction by leaving more space between active pixels (Section \ref{blk_prune}); \textbf{(3)} further smoothing masks with $2\pi$ periodic phase modulation. 
% Our methods could significantly reduce the roughness score on various datasets,
% by 
% $35.7\%$, $34.2\%$, $28.1\%$ and $27.3\%$, on MNIST, FMNIST, KMNIST, EMNIST,
% % Results show that our physics-aware roughness optimization can provide 
% % $35.7\%$, $34.2\%$, $28.1\%$, and $27.3\%$ reduction in roughness with minor accuracy loss, and $40\%$, $50.6\%$, $37.4\%$, and $35.7\%$ reduction in roughness
% % % with minor accuracy drop 
% % with intra-block smoothness 
% % on MNIST, FMNIST, KMNIST, and EMNIST,
% respectively,
Our work outperforms existing approaches~\cite{lin2018all,zhou2021large,li2022physics} for two reasons. First, \cite{lin2018all} did not model the interpixel crosstalk in DONN, therefore is roughness oblivious. Our work, however, integrates the interpixel crosstalk impact into the DONN loss function to be accuracy awareness \cite{lou2023effects}.
Second, previous studies~\cite{zhou2021large,li2022physics} leverage the periodic characteristic of phase modulation for deploying negative phase parameters on existing hardware, i.e., phase modulation is physically equivalent by adding $2\pi$ or its multiple. However, this periodic characteristic has not yet being explored in reducing interpixel crosstalk impacts.
% (@shanglin: check the numbers)}

% , which combines roughness modeling regularization with physics-aware weight sparsification to reduce the interpixel interaction within the phase mask in DONN system. Specifically, our proposed physics-aware optimization process includes three steps (Table \ref{tbl:pruning_feature}): \textbf{(1)} integrating roughness regularization into DONN loss function during the DONN training process. Details are illustrated in Section \ref{roughness}, where a regularization factor is introduced in the training loss for the roughness-aware DONN training; \textbf{(2)} compressing models with block sparsification to introduce mask sparsity, which migrate interpixel interaction by leaving more space between active pixels (Section \ref{blk_prune}); \textbf{(3)} further smoothing masks with $2\pi$ periodic phase modulation. As illustrated in Section \ref{smooth}, by taking advantage of the $2\pi$ period in phase changes, we can further smooth the mask w.r.t the pruned blocks and the active pixels. With Gumbel-Softmax for selecting the add-on phase with {0, $2\pi$} for each individual phase mask, the mask roughness can be further reduced without model performance degradation. 


\begin{table}[t]
%\tiny
\caption{Comparison of different methodologies.}
\label{tbl:pruning_feature}
\centering
\begin{adjustbox}{width=0.93\columnwidth, center}
\begin{tabular}{c|ccc}
\toprule
\textbf{Methods} & \multicolumn{1}{c}{\bf Roughness-aware} & \multicolumn{1}{c}{\bf Sparsity} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf 2$\pi$~Periodic} \\ {\bf Optimization}\end{tabular}} \\ 
\toprule
\cite{lin2018all,mengu2020scale}                  & \ding{53}  & \ding{53}  &  \ding{53} \\ 
\midrule
\cite{zhou2021large,li2022physics} & \ding{53}  & \ding{53}  & \checkmark \\ 
\midrule
%Ours                               & \checkmark & \ding{53}  & \ding{53}  \\ 
%\midrule
%Ours                               & \checkmark & \checkmark & \ding{53}  \\ 
%\midrule
Ours                               & \checkmark & \checkmark & \checkmark \\ 
\toprule
\end{tabular}
\end{adjustbox}
% \vspace{-0.7cm}
\end{table}
%Specifically, we proposed roughness modeling during DONN training process by integrating roughness regularization into DONN loss function. Sharp phase changes between neighboring pixels in phase masks can be reduced. Moreover, we leverage the block pruning method to introduce sparsity into diffractive layers for the purpose of reducing functioning diffraction pixels and leaving more space in the phase mask. Based on the $2\pi$ periodic feature for the phase modulation of the optical signal, we further propose a $2\pi$ post-smoothing method through Gumbel-Softmax to to reduce the roughness and preserve the smoothness of the phase masks in DONN.

% {\color{red}add concluded contributions@Shanglin}

Our contributions are summarized as follows:
\begin{itemize}
\item We propose a physics-aware roughness optimization framework, which integrates roughness modeling and weight sparsification into DONN training process, to effectively narrow the performance mismatch between digitally emulated DONN and physical hardware deployment.
    
\item We propose a roughness modeling method, 
% that integrate roughness regularization into DONN loss function,
which smooths the phase masks in DONNs training and also provides a method to quantify the performance gap.

\item We leverage the physics-aware block sparsification method into the optimization process to introduce sparsity of the DONN system and reduce the
interpixel interactions.

\item We apply $2\pi$ periodic phase modulation to further smooth the phase masks and reduce the performance mismatch.
\end{itemize}


% As illustrated in Section \ref{smooth}, by taking advantage of the $2\pi$ period in phase changes, we can further smooth the mask w.r.t the sparsified blocks and the active pixels. With Gumbel-Softmax for selecting the add-on phase with {0, $2\pi$} for each individual phase mask, the mask roughness can be further reduced without model performance degradation. 
Evaluation results demonstrate that our proposed physic-aware optimization framework provides up to $35.7\%$ 
% (\textcolor{red}{(how do we get this number?)})
reduction in roughness.
% with minor or even no accuracy loss. 
To the best of our knowledge, this is the first work to address the performance \textit{mismatch} between digital emulation and hardware deployment of DONNs.

==> mnist_DE.tex <==
% \begin{figure}[!htb]
%      \centering
%      \begin{subfigure}[b]{0.4\linewidth}
%          \centering       
%          \includegraphics[width=0.7\linewidth]{DAC23 -- DONN/fig/Pareto.pdf}
%          \caption{Pareto frontiers.}
%          \label{Pareto}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.4\linewidth}
%          \centering
%          \includegraphics[width=0.7\linewidth]{DAC23 -- DONN/fig/prune_DE.pdf}
%          \caption{Selection on pruning ratio.}
%          \label{prune_DE}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.4\linewidth}
%          \centering
%          \includegraphics[width=0.7\linewidth]{DAC23 -- DONN/fig/rough_DE.pdf}
%          \caption{Selection on regularization of roughness.}
%          \label{rough_DE}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.4\linewidth}
%          \centering
%          \includegraphics[width=0.7\linewidth]{DAC23 -- DONN/fig/intra_DE.pdf}
%          \caption{Selection on regularization of intra-block smoothness.}
%          \label{fig:intra_DE}
%      \end{subfigure}
% \caption{}
% \label{fig:DE}
% \end{figure}


% -------------------
\begin{figure}[t]
\centering
  \includegraphics[width=\linewidth]{fig/DE_plot.pdf}
\vspace{-0.7cm}
\caption{Hyperparameter Exploration. (a) Pareto frontiers of accuracy vs. roughness score of explorations on MNIST. (b) - (d) Exploration of sparsification ratio, regularization of roughness and intra-block smoothness vs. accuracy and roughness score. %{\color{red}@shanglin, the font size is too small (cunxi)} 
}
\label{DE_plot}
% \vspace{-0.2cm}
\end{figure}
% -------------------

We 
% collect the explored solutions from the MNIST dataset to form the results of
further perform
hyperparameter exploration in Fig.~\ref{DE_plot}. Fig.~\ref{DE_plot} (a) shows the Pareto frontier for roughness score vs. accuracy. It is clear that as the accuracy increases, the roughness score increases accordingly, which means the performance mismatch between digital emulation and hardware deployment of DONN system would be larger. In this case, hyperparameters need to be adjusted to address this trade-off. For Fig.~\ref{DE_plot}(b)-(d), we further explore the relation of accuracy and roughness score vs. sparsification ratio and regularizations of roughness and intra-block smoothness. We observe that accuracy and roughness score both decrease but under different magnitudes as the sparsification ratio and regularization increase. For roughness regularization in Fig.~\ref{DE_plot}(c), both accuracy and roughness score show an inflection point at $0.1$, with accuracy subsequently showing a rapid decrease, and roughness becomes smoother. Similarly for intra-block regularization in Fig.~\ref{DE_plot}(d), the inflection point is shown when the $\log$ of regularization is $1$. We also observe that these trends hold for the other three datasets.



==> onn.tex <==
There are three components (Fig. \ref{fig:donn_system}(a)) in a DONN system: (1) laser source for input images encoding, (2) diffractive layers for providing trainable phase modulation, and (3) detectors for capturing the diffraction pattern of the forward propagation. Specifically, the input image is first encoded with the coherent laser light. The information-encoded light signal is diffracted in the free space between diffractive layers, and modulated via phase modulation at each layer. Finally, the diffraction pattern after light propagation w.r.t light intensity distribution is captured at the detector plane for predictions. 

% From the beginning of the system, 
The input (e.g., an image) is encoded on the coherent light signal from the laser source, its wavefunction can be expressed as $f_{0}(x_{0}, y_{0})$. The wavefunction after light diffraction over diffraction distance $z$ to the first diffractive layer
% can be seen as 
is the summation of the outputs at the input plane, % \textcolor{red}{(where is it in Fig. 1?)}, 
i.e., 
\begin{equation}
\label{eq:diffraction_time}
    f_{1}(x, y) = \iint f_{0}(x_{0}, y_{0})h(x-x_{0}, y-y_{0}, z)dx_{0}dy_{0}
\end{equation}
where $(x, y)$ is the coordinate on the receive plane. 
% \textcolor{red}{(where is it in Fig. 1?)}. 
$h$ is the impulse optical response function of free space, which is the mathematical approximation for light diffraction, e.g., Rayleigh-Sommerfeld approximation, Frensel approximation, Frauhofer approximation~\cite{tobin1997introduction}.
% , resulting in the non-trainable parameters in DONN systems. 

 Equation \ref{eq:diffraction_time} can be calculated with spectral algorithm, where we employ Fast Fourier Transform (FFT) for fast and differentiable computation, i.e., 
% \begin{equation}
% \label{equ:diffraction_freq}
    $U_{1}(\alpha, \beta) = U_{0}(\alpha, \beta)H(\alpha, \beta, z)$,
% \end{equation}
where $U$ and $H$ are the Fourier transformation of $f$ and $h$ respectively. 
%The impulse function used for Fresnel approximation is 
%\begin{equation}
%\label{eq:diffraction_time_end}
%    h(x, y, z) = \frac{\exp(ikz)}{i\lambda z}\exp\{\frac{ik}{2z}(x^{2} + y^{2})\}
%\end{equation}
%where $i=\sqrt{-1}$, $\lambda$ is the wavelength of the laser source, $k=2\pi/\lambda$ is free-space wavenumber.
% After light diffraction, 
The
% resulting 
wavefunction
% in Equation \ref{equ:diffraction_freq} 
$U_{1}(\alpha, \beta)$ is transformed to time domain with inverse FFT (iFFT) for phase modulation:
% , and the phase modulation 
% $W(x, y)$. 
% provided by the diffractive layer is applied to the light wavefunction by matrix multiplication, i.e.,
% \begin{equation}
% \label{eq:phase_mod}
    $f_{2}(x, y) = \text{iFFT}(U_{1}(\alpha, \beta)) \times \mathbf{W}_{1}(x, y)$,
% \end{equation}
where $\mathbf{W}_{1}(x, y)$ is the phase modulation in the first diffractive layer. 
$f_{2}(x, y)$ is the 
% input light 
wavefunction for the light diffraction for the second diffractive layer. 

We wrap one computation round of light diffraction and phase modulation at one diffractive layer as a computation module named \textbf{DiffMod}, i.e.,
% \begin{equation}
% \label{eq:diffmod}
    $\text{DiffMod}(f(x, y), \mathbf{W}) = L(f(x, y), z) \times \mathbf{W}(x, y)$,
% \end{equation}
where $f(x, y)$ is the input wavefunction.
$\mathbf{W}(x, y)$ is the phase modulation. 
$L(f(x, y), z)$ is the wavefunction after light diffraction over a constant distance $z$ in time domain.  
% As a result, 
% In a multiple diffractive layer constructed DONN system, the forward function can be computed iteratively for the stacked diffractive layers. For example, 
For a 3-layer DONN system,
% shown in Figure \ref{fig:donn_system}, 
the forward function can be expressed as,
\begin{equation}
\label{eq:forward}
\small
\begin{split}
I(f_{0}(x, y), \mathbf{W}) = \text{DiffMod}(\text{DiffMod}(\text{DiffMod}(f_{0}(x, y), \\
\mathbf{W}_{1}(x, y)),\mathbf{W}_{2}(x, y)), \mathbf{W}_{3}(x, y))
\end{split}
\end{equation}
The final diffraction pattern w.r.t the light intensity $I$ in Equation \ref{eq:forward} is captured at the detector plane. 
% (where is it in Fig. 1?). 
There are pre-defined detector regions
% on the detector plane 
to mimic the output of conventional neural networks for class prediction. The class with the highest sum of light intensity within its corresponding detector region produced by \texttt{argmax} is picked as the prediction result~\cite{lin2018all,li2020multi}.
Suppose
% the one-hot represented 
the ground truth class $t$, the loss function $\boldsymbol\ell$
% can be acquired with 
using \textbf{MSELoss} is
% \begin{equation}
% \label{mse}
    $\boldsymbol\ell = \parallel \text{Softmax}(I) - t \parallel_{2}$.
% \end{equation}
% \textcolor{red}{(t should change format)}
%As proposed in~\cite{lin2018all,li2020multi}, the output plane is divided into \textbf{ten} detector regions to mimic the output of conventional neural networks for predicting \textbf{ten} classes. The final class will be produced by \texttt{argmax} function with the ten intensity sums of the ten detector regions as input. For example, in Figure \ref{fig:system}, based on the label indices of the ten detector regions for image "2", we can see that the 3$^{rd}$ region on the first row has the highest energy. Then, the predicted class is class "2". Similarly, the predicted classes "1", "8", and "9" of other three datasets can be generated by applying \texttt{argmax} on the detector. With the one-hot represented ground truth class $t$, the loss function $L$ can be acquired with \textbf{MSELoss} as,
%\begin{equation}
%    L = \parallel \text{Softmax}(I) - t \parallel_{2}
%\end{equation}
Thus, the whole system is designed to be differentiable and compatible with conventional automatic differential engines.


==> pruning.tex <==



\begin{figure}[t]
\centering
  \includegraphics[width=0.9\linewidth]{fig/prune.pdf}
\vspace{-0.1cm}
\caption{Comparison of block sparsification with two other sparsification methods. All three are with sparsification ratio being 0.33.}
\label{prune}
\vspace{-0.1cm}
\end{figure}

\vspace{-0.1cm}
\subsubsection{Roughness-Aware Sparsification}

To consider the case of different sparsification methods (i.e., bank balanced sparsity, irregular sparsity, and block sparsity), Fig.~\ref{prune} shows the roughness impact using same sparsity ratio (i.e., $0.33$).
% but different sparsities types . 
Roughness is computed based on Equation~\ref{rough_score} with $8$-neighbors.
% mitigates roughness score.
% compares the block sparsification with other commonly used sparsification methods. 
% Given the $0.33$ sparsification ratio, the weight matrix is pruned under different patterns under the three methods, 
For the block sparsification (Fig.~\ref{prune}(a)), we partition the weight matrix into equal-sized blocks. 
% $L_2$-norm is computed for each of the block. 
Based on the pre-defined threshold or percentile, all the weights within the blocks with the $L_2$-norm smaller than the threshold or the percentile are set to zero. 
For the non-structured sparsification (Fig.~\ref{prune} (b)), weights with absolute value that is smaller than the pre-defined threshold or percentile are sparsified~\cite{han2015learning}. For the bank-balanced sparsification (Fig.~\ref{prune}(c)), rows of weight matrix are split into equal-sized banks, and identical sparsity among banks is kept while sparsification~\cite{cao2019efficient}.
% Compared with the other two methods, 
Among all, block sparsification focuses more on the whole blocks of the weight rather than the element-wise pattern, which leads to the lowest roughness.
% As some blocks in the weight matrix are pruned, values in these blocks would be set to zero, which means the roughness within these blocks are zero, and therefore the smoothness of the weight matrix will increase accordingly.

\subsubsection{SLR-Regularized Optimizations}
We integrate the block weight sparsification method~\cite{lagunas2021block} with the Surrogate Lagrangian Relaxation (SLR)-based model compression optimization technique~\cite{gurevin2020enabling} to reduce functioning diffraction pixels and further achieve smoothness of the phase masks in DONN (Fig.~\ref{fig:donn_system}(c)).
For a DONN with $N$ layers, as $i \in 1,2,...,N$, denote the weights of each diffractive layer as $\mathbf{W}_i$. The objective of our block sparsification is to minimize the DONN loss function (Equation~\ref{rough_loss}) while reducing the number of non-zero blocks of weights in each $\mathbf{W}_i$, i.e., 
% $\min_{\mathbf{W}_i} L(\mathbf{W}_i)$, 
$\min_{\mathbf{W}_i} \{\boldsymbol\ell(\mathbf{W}_i) + 
% p\times R(\mathbf{W}_i)\}
\boldsymbol\ell_{r}(\mathbf{W}_i)\}$
subject to \ding{172} \# non-zero block rows in $\mathbf{W}_i$ is less than $r_i$ and \ding{173} \# non-zero block columns in $\mathbf{W}_i$ is less than $c_i$, where $r_i$ and $c_i$ are the desired non-zero block of rows and columns respectively, and $i = 1, ..., N$.
% $\boldsymbol\ell(\mathbf{W}_i)$ is the MSELoss in Eq.~\ref{mse}, $\boldsymbol\ell_{rough}(.)$ is the roughness regularizer. 
The unconstrained form can be written as Equation~\ref{relax}.
\vspace{-0.3cm}
\begin{equation}
\small
\begin{aligned}
\label{relax}
&\min_{\mathbf{W}_i}\boldsymbol\ell(\mathbf{W}_i) + 
% p\times R(\mathbf{W}_i)
\boldsymbol\ell_{r}(\mathbf{W}_i)
+ \sum_{i=1}^N g_i\left(\mathbf{W}_i\right) \\
\text{where} &\;
g_{i}\left(\mathbf{W}_{i}\right)=\left\{\begin{array}{ll}
0 & \text { if \ding{172} and \ding{173} are satisfied}  \\
+\infty & \text { otherwise }
\end{array}\right.
\end{aligned}
\vspace{-0.2cm}
\end{equation}
% In the equation, 
$\boldsymbol\ell(.) + 
% p\times R(.)
\boldsymbol\ell_{r}(.)$ represents the DONN system loss with roughness regularization. $g_i(.)$ is the indicator function that represents the non-differentiable penalty term for each diffractive layer. To solve this,
% 
% the SLR-based sparsification optimization technique
 the duplicate variables $\mathbf{Z}_i$ is introduced~\cite{boyd2011distributed,gurevin2020enabling}.
%  for the decomposition of 
%  to decompose the loss function into smaller subproblems~\cite{boyd2011distributed}. 
 The loss function is equivalent as: $\min_{\mathbf{W}_i} \{\boldsymbol\ell(\mathbf{W}_i) + 
% p\times R(\mathbf{W}_i) 
\boldsymbol\ell_{r}(\mathbf{W}_i) + \sum_{i=1}^N g_{i}(\mathbf{Z}_i)\}, \: s.t. \: \mathbf{W}_i = \mathbf{Z}_i, i = 1, ..., N$. The resulting Augmented Lagrangian function is 
% can be written as Equation~\ref{Aug}.  
\vspace{-0.2cm}
\begin{equation}
\label{Aug}
\small
\begin{aligned}
\mathcal{L} \left(\mathbf{W}_i, \mathbf{Z}_i, \mathbf{\Lambda}_i\right) & = 
\boldsymbol\ell(\mathbf{W}_i) + 
\boldsymbol\ell_{r}(\mathbf{W}_i) + \sum_{i=1}^N g_i\left(\mathbf{Z}_i\right) \\
&+\sum_{i=1}^N \operatorname{tr}\left[\mathbf{\Lambda}_i^T\left(\mathbf{W}_i-\mathbf{Z}_i\right)\right]+\sum_{i=1}^N \frac{\rho}{2}\left\|\mathbf{W}_i-\mathbf{Z}_i\right\|_F^2
\end{aligned}
\vspace{-0.2cm}
\end{equation}
Here, $\mathbf{\Lambda}_i$ are Lagrangian multipliers for relaxing the constraints. Their violations are penalized by quadratic penalties with coefficient $\rho$. $\|\cdot\|_F$ is the Frobenius norm. $tr(.)$ is the trace.
We could decompose the above problem into
% This relaxed problem then can be decomposed into 
two subproblems and solve them iteratively until convergence. At iteration $k$, the first subproblem is: given $\mathbf{\Lambda}_i^k$ and $\mathbf{Z}_i$ from the previous iteration, solving the loss function $\min_{\mathbf{W}_i}\mathcal{L}\left(\mathbf{W}_i, \mathbf{Z}_i^{k-1}, \mathbf{\Lambda}_i^k\right)$. At this time, we check the surrogate optimality condition $\mathcal{L}\left(\mathbf{W}_i^k, \mathbf{Z}_i^{k-1}, \mathbf{\Lambda}_i^k\right)<\mathcal{L}\left(\mathbf{W}_i^{k-1}, \mathbf{Z}_i^{k-1}, \mathbf{\Lambda}_i^k\right)$. If 
% this condition is 
satisfied, $\mathbf{\Lambda}_i^k$ would be updated as $\mathbf{\Lambda^\prime}_i^{k} = \mathbf{\Lambda}_i^k+s^{\prime k}\left(\mathbf{W}_i^k-\mathbf{Z}_i^{k-1}\right)$. The second subproblem is: fixing $\mathbf{W}_i^k$ from the first subproblem, solving the loss function $\min_{\mathbf{Z}_i}\mathcal{L}\left(\mathbf{W}_i^k, \mathbf{Z}_i, \mathbf{\Lambda^\prime}_i^{k}\right)$. Similar,  we need to check the surrogate optimality condition $\mathcal{L}\left(\mathbf{W}_i^k, \mathbf{Z}_i^k, \mathbf{\Lambda^\prime}_i^{k}\right) < \mathcal{L}\left(\mathbf{W}_i^k, \mathbf{Z}_i^{k-1}, \mathbf{\Lambda^\prime}_i^{k}\right)$ to update $\mathbf{\Lambda}_i^{k+1} = \mathbf{\Lambda^\prime}_i^k+s^k\left(\mathbf{W}_i^k-\mathbf{Z}_i^{k}\right)$. Both $s^{\prime k}$ and $s^{k}$ are stepsize~\cite{gurevin2020enabling}.

==> result.tex <==
% In this part, 
We present the results of applying our proposed physics-aware roughness optimization to the four datasets.
In all the experiments, \textbf{Ours-A} refers to the roughness-aware trained model; \textbf{Ours-B} refers to the model trained with sparsity; \textbf{Ours-C} refers to the model trained with sparsity and roughness; \textbf{Ours-D} refers to the model trained with sparsity, plus roughness and intra-block smoothness. The system roughness score is calculated as the average of the roughness of all phase masks: $R_{overall} = \overline{R(\mathbf{W})}$, where $R(\mathbf{W})$ is from Equation~\ref{rough_score}. 
$R_{overall}$ quantifies the overall interpixel interaction within all the phase masks in a DONN system. A lower score means weaker interpixel interaction and less mismatch between numerical modeling and practical deployment.

% ------------------------------------
% \subsubsection{MNIST}

\begin{table}[t]
\caption{MNIST Result. Baseline is trained under $50$ epochs. The sparsification are trained with block size equal to $25$.}
\label{mnist}
\centering
\begin{adjustbox}{width=\columnwidth, center}
\scriptsize
\begin{tabular}{c|c|cc}
\toprule
\textbf{Model} & 
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}{\bf Accuracy} \\ {\bf (\%)}\end{tabular}} & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf $R_{overall}$ before} \\ {\bf $2\pi$ optimization }\end{tabular}} & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf $R_{overall}$ after} \\ {\bf $2\pi$ optimization }\end{tabular}} \\
\midrule
\cite{lin2018all, zhou2021large,li2022physics} & 96.67 & 466.39 & 460.85 \\
% \cite{zhou2021large,li2022physics} & xx & xx & xx \\
\midrule
Ours-A & 96.18 & 416.07 & -- \\
Ours-B & 96.38 & 538.78 & 400.38 \\ 
Ours-C & 96.47 & 409.41 & 299.87 \\
Ours-D & 95.90 & 375.35 & \textbf{280.32} \\
\toprule
\end{tabular}
\end{adjustbox}
% \vspace{-0.3cm}
\end{table}

% ------------------------------------
% \subsubsection{FMNIST}

\begin{table}[t]
\caption{FMNIST Result. Baseline is trained under $150$ epochs. The sparsification are trained with block size equal to $20$.}
\label{fmnist}
\centering
\begin{adjustbox}{width=\columnwidth, center}
\scriptsize
\begin{tabular}{c|c|cc}
\toprule
\textbf{Model} & 
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}{\bf Accuracy} \\ {\bf (\%)}\end{tabular}} & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf $R_{overall}$ before} \\ {\bf $2\pi$ optimization }\end{tabular}} & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf $R_{overall}$ after} \\ {\bf $2\pi$ optimization }\end{tabular}} \\
\midrule
\cite{lin2018all,zhou2021large,li2022physics} & 87.98 & 464.78 & 461.98 \\
% \cite{zhou2021large,li2022physics} & xx & xx & xx \\
\midrule
Ours-A & 86.99 & 421.49 & -- \\
Ours-B & 87.88 & 488.11 & 438.53 \\ 
Ours-C & 86.79 & 350.67 & 305.86 \\
Ours-D & 85.76 & 450.73 & \textbf{229.70} \\
\toprule
\end{tabular}
\end{adjustbox}
% \vspace{-0.3cm}
\end{table}

% ------------------------------------
% \subsubsection{KMNIST}

\begin{table}[t]
\caption{KMNIST Result. Baseline is trained under $100$ epochs. The sparsification are trained with block size equal to $20$.}
\label{kmnist}
\centering
\begin{adjustbox}{width=\columnwidth, center}
\scriptsize
\begin{tabular}{c|c|cc}
\toprule
\textbf{Model} & 
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}{\bf Accuracy} \\ {\bf (\%)}\end{tabular}} & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf $R_{overall}$ before} \\ {\bf $2\pi$ optimization }\end{tabular}} & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf $R_{overall}$ after} \\ {\bf $2\pi$ optimization }\end{tabular}} \\
\midrule
\cite{lin2018all,zhou2021large,li2022physics} & 86.92 & 460.61 & 445.57 \\
% \cite{zhou2021large,li2022physics} & xx & xx & xx \\
\midrule
Ours-A & 85.26 & 462.7 & -- \\
Ours-B & 86.83 & 473.08 & 432.26 \\ 
Ours-C & 85.01 & 396.84 & 331.22 \\
Ours-D & 83.19 & 327.48 & \textbf{288.42} \\
\toprule
\end{tabular}
\end{adjustbox}
% \vspace{-0.3cm}
\end{table}

% ------------------------------------
% \subsubsection{EMNIST}

\begin{table}[t]
\caption{EMNIST Result. Baseline is trained under $100$ epochs. The sparsification are trained with block size equal to $20$.}
\label{emnist}
\centering
\begin{adjustbox}{width=\columnwidth, center}
\scriptsize
\begin{tabular}{c|c|cc}
\toprule
\textbf{Model} & 
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}{\bf Accuracy} \\ {\bf (\%)}\end{tabular}} & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf $R_{overall}$ before} \\ {\bf $2\pi$ optimization }\end{tabular}} & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}{\bf $R_{overall}$ after} \\ {\bf $2\pi$ optimization }\end{tabular}} \\
\midrule
\cite{lin2018all,zhou2021large,li2022physics} & 92.30 & 463.42 & 458.48 \\
% \cite{zhou2021large,li2022physics} & xx & xx & xx \\
\midrule
Ours-A & 91.61 & 435.58 & -- \\
Ours-B & 92.36 & 465.85 & 443.91 \\ 
Ours-C & 91.16 & 349.61 & 336.75 \\
Ours-D & 90.74 & 312.17 & \textbf{298.09} \\
\toprule
\end{tabular}
\end{adjustbox}
% \vspace{-0.5cm}
\end{table}

% ---------------------

% MNIST is handwritten digits database with $60,000$ examples as training set and $10,000$ as testing set. 
Table~\ref{mnist}, \ref{fmnist}, \ref{kmnist} and \ref{emnist} compare the accuracy and roughness score of each component of our proposed optimization method on the four datasets.
For all the experiments,  \cite{lin2018all} has the highest roughness score.
% , the highest classification accuracy, it is also accompanied by the highest roughness score.
With the $2\pi$ optimization, the roughness score dropped less than $2\%$, which means the phase change between pixels in the phase masks is very drastic within $2\pi$ range. 
The roughness-aware training (Ours-A) results to around $10\%$ roughness drop but still with relatively high roughness score. The sparsification (Ours-B) results to higher accuracy compared with roughness-aware training but also higher roughness score because of the sharp phase changes between sparsified pixels and their surroundings as explained in Section~\ref{post_smooth}. With the help of $2\pi$ optimization, the phase gap is smoothed with the $2\pi$ periodic feature and the roughness score dropped to the same level as of roughness-aware training. 
Hence, the combination of the sparsification and the roughness modeling (Ours-C) shows great improvement. It results to the drop of the roughness score in $12.2\%$, $24.6\%$, $13.8\%$ and $24.6\%$ respectively for the four datasets before the $2\pi$ optimization, $35.7\%$, $34.2\%$, $28.1\%$ and $27.3\%$ after the $2\pi$ optimization, with little impact on accuracy.
The introduction of intra-block smoothness (Ours-D) further reduces the roughness score. Given a bit more accuracy flexibility (in average 2\% acorss all datasets), we reduce the roughness after $2\pi$ optimization by $40\%$, $50.6\%$, $37.4\%$ and $35.7\%$ for the four datasets, respectively.

% -------------------
% \begin{figure*}[!ht]
% \centering
%   \includegraphics[width=0.9\linewidth]{fig/map_1.pdf}
% \caption{Comparison of the phase mask of the second diffractive layer under EMNIST dataset. The first and the second row are phase masks before and after the $2\pi$ optimization. The black blocks mean that the weights inside are pruned and set to zero. {\color{red}@shanglin, I suggest to keep first row and the last image in the 2nd row (cunxi)} }
% \label{map}
% \end{figure*}


Fig.~\ref{map} compares the second phase mask (diffractive layer) of DONN in different models under the EMNIST dataset. 
% The first rows are phase masks before the $2\pi$ optimization. The black blocks are the pruned areas and weights inside are zeros, which form sharp contrast with the surrounding colors. The second row shows the phase masks after the $2\pi$ post-smooth optimization. With the selectively addition of $2\pi$ to each pixel in the entire phase mask, the previous black areas blend in with the surrounding color and the entire masks become smoother. 
The first four are phase masks without the $2\pi$ optimization. The black blocks are the sparsified areas,
% and weights inside are zeros, 
which form sharp contrast with the surrounding colors. The last is the phase mask from the model trained with sparsity, roughness and intra-block smoothness and with $2\pi$ post-smooth optimization applied.
With the selectively addition of $2\pi$ to each pixel in the entire phase mask, the previous black areas blend in with the surrounding color and the entire masks become smoother.
Moreover, with the awareness of the mask roughness during training, the valid phase modulations in diffractive layers are more clustered at the center part of the mask while the edge part is more likely to provide marginal modulations.
% With more roughness awareness for the DONN design, 
% The valid pattern gets more clustered and the mask is overall more smooth.
This correlates with the optical characteristics where the light signal strength decays from the center. Thus, the most valid information and phase modulation are expected to happen at the center of the mask. The smoothed phase mask will result in easy fabrication of the mask and better correlation for DONN numerical modelling and its physical deployment.
%\textcolor{red}{@Yingjie. Please add some physical insight on comparison of four masks in second row.}



==> roughness.tex <==
\begin{figure}[b]
     \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering       \includegraphics[width=0.45\linewidth]{DAC23 -- DONN/fig/rough_4.pdf}
         \caption{
        %  Roughness modelling with 
         4-neighbors.}
         \label{fig:rough_4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
      \includegraphics[width=0.45\linewidth]{DAC23 -- DONN/fig/rough_8.pdf}
         \caption{
        %  Roughness modelling with 
         8-neighbors.}
         \label{fig:rough_8}
     \end{subfigure}
        \caption{Illustration of roughness modelling for a phase mask with size of $3\times3$ -- (a) with 4 neighbors, (b) with 8 neighbors. }
        \label{fig:rough}
% \vspace{-0.5cm}
\end{figure}



% We first define the roughness score.

% By reducing the roughness of the mask, the incident field varies smoothly, which maintains its consistency with the optical response computed in the training process. 

We develop the the roughness modelling applicable independently for each diffractive layer and differentiable with the training process, targeting the roughness-aware training of the DONN model.
% is proposed in this Section. 
As shown in Fig. \ref{fig:rough}, the roughness of the pixel is computed with the values of its neighboring pixels. 
% Specifically, 
% We have 
% Two possible implementations are 4-neighbors and 8-neighbors. 
The one-dimension zeros padding is applied to the original phase mask for roughness computation of pixels at the boundary.
We average the $L_2$-norm differences of value at the pixel and values of its neighbors as the roughness at the pixel. For example, the roughness of the pixel $p_{11}$ in Fig. \ref{fig:rough}, the $k$-neighbor roughness is computed as
\begin{equation}
\small
    R(p_{11}) = \frac{1}{k} \times \Sigma_{ij} \parallel p_{ij} - p_{11} \parallel_{2}, p_{ij} \in \text{neighbor}(p_{11}) 
\end{equation}
where $k$ can be 4 or 8.
% in our implementation,
For 4-neighbors (Fig. \ref{fig:rough_4}), $\text{neighbor}(p_{11}) = \{p_{01}, p_{10}, p_{12}, p_{21}\}$; and for 8-neighbor roughness (Fig. \ref{fig:rough_8}), $\text{neighbor}(p_{11}) = \{p_{00}, p_{01}, p_{02}, p_{10}, p_{12}, p_{20}, p_{21}, p_{22}\}$.
% For boundary pixels, e.g., $p_{00}$, its 4-neighbor roughness is computed with neighbors of  $\{0, 0, p_{01}, p_{10}\}$. 
The roughness of the whole phase mask can be computed with the summation of the roughness of each pixel, i.e., 
\begin{equation}
\label{rough_score}
\small
    R(\mathbf{W}) = \Sigma_{ij} R(p_{ij}), i\in[0, N-1], j\in[0, N-1]
\end{equation}
where the phase mask $\mathbf{W}$ has the size of $N\times N$.
We sum up the roughness of all pixels as the roughness score of the diffractive layer.
% The roughness of all pixels within the diffractive layer are summed up as the roughness of the diffractive layer. 
We further integrate the roughness matrix
% The roughness matrix can also be 
% integrated 
into training,
% by adding the roughness to the system loss function,
i.e., 
\begin{equation}
\label{rough_loss}
\small
    L = \parallel \text{Softmax}(I) - t \parallel_{2} + p \times R(\mathbf{W}) % = \boldsymbol\ell(W) + p \times R(W)
\end{equation}
where $p$ is the regularization factor and $R(\mathbf{W})$ is the roughness results for each diffractive layer. 


% \textcolor{red}{(Training framework vs inference framework?)}
